How to morph planar graph drawings

Given an $n$-vertex graph and two straight-line planar drawings of the graph that have the same faces and the same outer face, we show that there is a morph (i.e., a continuous transformation) between the two drawings that preserves straight-line planarity and consists of $O(n)$ steps, which we prove is optimal in the worst case. Each step is a unidirectional linear morph, which means that every vertex moves at constant speed along a straight line, and the lines are parallel although the vertex speeds may differ. Thus we provide an efficient version of Cairns' 1944 proof of the existence of straight-line planarity-preserving morphs for triangulated graphs, which required an exponential number of steps.

==> abstract.tex <==
\begin{abstract}
\todo{update needed}
 % \small\baselineskip=9pt 
In 1944, Cairns proved the following theorem: given any two straight-line
planar drawings of a triangulation with the same outer face,
there exists a morph (i.e., a continuous transformation) between the two
drawings so that the drawing remains straight-line planar at all times. 
Cairns's original proof required exponentially many morphing steps. 
We prove that there is a morph that consists of $O(n^2)$ steps, where each step
is a linear morph  that moves each vertex at constant speed along a straight
line.


Using a known result on  compatible triangulations this implies that
for a general planar graph $G$ and any two straight-line planar drawings of $G$
with the same embedding, there is a morph between the two drawings that
preserves straight-line planarity and consists of $O(n^4)$ steps.
\end{abstract}


% the following comes from GD
%
%
%
% \begin{abstract}
% A morph between two straight-line planar drawings\remove{with the same outer
% face} of the same graph is a continuous transformation from the first to the
% second drawing such that planarity is preserved at all times. Each step of the
% morph moves each vertex at constant speed along a straight line. Although the
% existence of a morph between any two drawings was established several
% decades ago, only recently it has been proved that a polynomial number of
% steps
% suffices to morph any two planar straight-line drawings. Namely, at SODA
% $2013$, Alamdari \emph{et al.}~\cite{aacdfl-mpgdpns-13-c} proved that any two
% planar straight-line drawings of a planar graph can be morphed in $O(n^4)$
% steps, while $O(n^2)$ steps suffice if we restrict to maximal planar graphs.
% 
% In this paper, we improve upon such results, by showing an algorithm to morph
% any two planar straight-line drawings of a planar graph in $O(n^2)$ steps;
% further, we show that a morph with $O(n)$ steps exists between any two planar
% straight-line drawings of a series-parallel graph.
% \end{abstract}

==> algorithm.tex <==
\section{Overview of the Algorithm}
\label{se:overview}

In this section we describe all the ingredients of our algorithm and how they fit together.

Our most basic building block is an algorithm to morph a triangulation so that a given quadrilateral formed by two adjacent triangles becomes convex.  One chord of the quadrilateral will lie inside the quadrilateral.  A necessary condition is that the other chord not be part of the triangulation.
Specifically, we solve the following problem:

\begin{problem}[Quadrilateral Convexification]
Given an $n$-vertex triangulation $\Gamma$ with triangular outer boundary and given a quadrilateral $abcd$ in $\Gamma$ with no vertex inside it  and such that neither $ac$ nor $bd$ is an edge outside of $abcd$ (i.e.,~$abcd$ does not have external chords), 
morph $\Gamma$ so that $abcd$ becomes convex while the outer boundary remains fixed.
\label{prob:quad-convex}
\end{problem}

We solve Quadrilateral Convexification in Section~\ref{sec:quad-convexification} giving the following result: 
%Let $Q(n)$ be the number of unidirectional morphing steps needed for Quadrilateral Convexification.  We will prove:

\def\quadconvex{Quadrilateral Convexification can be solved via a morph composed of \update{$O(1)$ unidirectional morphs}.  Furthermore, 
such a morph can be found in $O(n^2)$ time.}
%there is an $O(n^2)$-time algorithm to find the morph.}
\begin{theorem}
\quadconvex
\label{thm:quad-convex}
\end{theorem}


We will prove our main result, Theorem~\ref{th:main}, by finding a morph that consists of 
$O(n)$ calls to Quadrilateral Convexification plus $O(n)$ further unidirectional morphs.
Together with the above Theorem~\ref{thm:quad-convex}, this gives a total bound of \update{$O(n)$ unidirectional morphs}.

%
%\begin{theorem}
%\label{thm:main-QC}
%Given a graph $G$ on $n$ vertices and two straight-line planar drawings of $G$ with the same faces and the same outer face, we can find in polynomial time 
%a morph between the two drawings that preserves straight-line planarity and consists of $O(nS_{\it QC}(n))$ unidirectional morphs.  \rednote{AL. Give time bound of algorithm.} 
%\end{theorem}
%

The proof of Theorem~\ref{th:main} has two parts.
In Section~\ref{sec:triangulate} we reduce the problem to the case of triangulations with the same outer triangular boundary.  Specifically, we show that given two topologically equivalent straight-line planar drawings of a graph $G$ on $n$ vertices, 
we can enclose each drawing with an identical triangle and then morph and add (the same) edges
%we can enclose each drawing with the same triangle and then morph and add edges (and no vertices) 
to triangulate both drawings, using \update{$O(n)$ unidirectional morphs} and keeping the triangular outer boundary fixed. Note that a morph between these augmented drawings provides a morph of the originals by ignoring the added edges.
  
In Section~\ref{sec:morph-triangulations} we prove Theorem~\ref{th:main} for the case of triangulations with the same outer boundary, using \update{$O(n)$ unidirectional morphs}. Thus the two sections together prove Theorem~\ref{th:main}.

In all cases when we say that we find a morph, we actually find a pseudomorph (as defined in the previous section) and rely on the following theorem (which is proved in Section~\ref{sec:geometry}) to convert the pseudomorph to a true morph:

\def\pseudomorph{Let $\Gamma_1$ and $\Gamma_2$ be two triangulations with the same triangular outer boundary that  are topologically equivalent drawings of an $n$-vertex maximal planar graph $G$.
Suppose that  there is a pseudomorph from $\Gamma_1$ to $\Gamma_2$ 
in which we contract an internal vertex $v$ of degree at most 5, perform $k$ unidirectional morphs, and then uncontract $v$.
Then there is a morph $\cal M$ from $\Gamma_1$ to $\Gamma_2$ that consists of $k+2$ unidirectional morphs.  Furthermore, given the sequence of $k+1$ drawings that define the pseudomorph, we can modify them to obtain the sequence of drawings that define $\cal M$ in $O(k+n)$ time.
%given the pseudomorph, we can construct $\cal M$ in $O(k)$ time. 
}
\begin{theorem}
\pseudomorph
\label{thm:pseudomorph}
\end{theorem} 


Note that although the proofs of Theorems~\ref{thm:quad-convex} and~\ref{thm:pseudomorph} are deferred until the last two sections of the paper, they come first in terms of the dependency of results. 




\remove{
\begin{algorithm}[tb]
\renewcommand{\thealgorithm}{\texttt{Morph}} 
\caption{\PROC{}{$\Gamma_s$,$\Gamma_t$}}\label{algo:morph}
\begin{algorithmic}[1]
\algsetup{indent=1em,linenosize=\small,linenodelimiter=.}
\medskip
\REQUIRE{$\Gamma_s$ and $\Gamma_t$ are two straight-line planar drawings of a connected plane graph $G$}\\
\medskip
\COMMENT{preprocessing}
\STATE{morph and augment so that both drawings are triangulations with fixed outer triangle (Section~\ref{sec:triangulate})}\\
\COMMENT{base case}
\IF{$G$ is a triangle}
\STATE{return the identity morph}\label{line:morph2}
\ENDIF\vspace{.3em}
\COMMENT{recursive step}
\STATE $v \gets$ an internal vertex of degree $\le 5$\label{line:morph4}
\STATE $u \gets$ a neighbor of $v$ to which $v$ can be contracted in $\Gamma_t$\label{line:morph5}
\STATE morph $\Gamma_s$ so that $v$ can be contracted to $u$ \label{line:morph6} 
\STATE $\Gamma_s^u \gets$ contract $v$ to $u$ in $\Gamma_1$\label{line:morph7}
\STATE $\Gamma_t^u \gets$ contract $v$ to $u$ in $\Gamma_2$\label{line:morph8}
\STATE ${\cal M} \gets$ {\sc Morph}$(\Gamma_s',\Gamma_t')$\label{line:morph9}\vspace{.3em}\\
\RETURN PseudoMorph-to-Morph(<$\Gamma_1, \Gamma_1^u$> $ {\cal M}$ <$\Gamma_2^u, \Gamma_2$ >)
\end{algorithmic}
\end{algorithm}
}





==> introduction-Anna.tex <==
\section{Introduction}\label{se:intro}

A morph between two geometric shapes is a continuous transformation of one shape into
the other. 
Morphs are useful in many areas of computer science---Computer Graphics, Animation, and Modeling, to name just a few.
%Computer Graphics, Animation, and Modeling are only few of the areas of Computer Science that make use of morphs.
The usual goal in morphing is to ensure that the structure of the shapes be ``visible'' throughout the entire transformation.

%Graph drawing has developed into a mature field with a rich mix of applications and theory.
%See the books~\cite{DETT,Kaufmann-Wagner} and the forthcoming handbook~\cite{handbook}.
%Recently, several papers have addressed the problem of \emph{morphing} graph drawings. 


Two-dimensional graph drawings can be used to represent many of the shapes for which morphs are of interest, e.g., two-dimensional
images~\cite{bn-fbim-92,fm-ffip-98,te-imfpt-99}, polygons, and  poly-lines~\cite{aadddhlrssw-cpwlv-11,acl-arpsi-00,cc-wgosm-97,elrsw-cssp-98,gh-msp-94,nmwb-mpstcg-08,sgwm-2dsbisvpp-93,sg-pba2dsb-92,sr-sbussr-95}. 
For this reason, morphs of graph drawings have been well studied. 

For the problem of morphing graph drawings,  
%In this context, 
the input consists of two 
drawings $\Gamma_1$ and $\Gamma_2$ of the same graph $G$, and the problem is to transform continuously from the first drawing to the second drawing.
%one drawing to the other. 
A \emph{morph} between $\Gamma_1$ and $\Gamma_2$ is  a continuously changing family of drawings of $G$ indexed by time $t \in  [0, 1]$, such that the drawing at time $t = 0$ is $\Gamma_1$ and the drawing at time $t = 1$ is $\Gamma_2$. 
%Preserving 
Maintaining structure during the morph becomes a matter of preserving geometric properties such as planarity, straight-line planarity, edge lengths, or edge directions.
For example, preserving edge lengths in a straight-line drawing leads to problems of linkage reconfiguration~\cite{CDR,DO'R}.

%{\smallskip\noindent\bf Morphing Planar Graph Drawings.}
In this paper we consider the problem of morphing between two graph drawings while preserving planarity.
Of necessity, we 
assume that the initial and final planar drawings are \emph{topologically equivalent}---i.e., have the same faces and the same outer face.
In addition to the above-mentioned applications, morphing graph drawings while preserving planarity has application to the problem of creating three-dimensional models from two-dimensional slices~\cite{BS}, with time playing the role of the third dimension.

When planar graphs may be drawn with poly-line edges the morphing problem becomes much easier---the intuition is that vertices can move around while edges bend to avoid collisions.  An efficient morphing algorithm for this case was given by 
Lubiw and Petrick~\cite{LP}. 
The case of orthogonal graph drawings is also well-solved---Biedl et al.~\cite{biedl2013morphing} gave
%a SODA'06 paper describes 
an algorithm to morph efficiently between any two orthogonal drawings of the same graph while preserving planarity and orthogonality.

%{\smallskip\noindent\bf Morphing Straight-Line Planar Drawings.}
We restrict our attention in this paper to straight-line planar drawings.
Our main result is an efficient algorithm to morph between two topologically equivalent straight-line planar drawings of a graph, where the morph must preserve straight-line planarity.  The issue is to find the vertex trajectories, since the edges are determined by the vertex positions.

%{\smallskip\noindent\bf Existence.}
Existence of such a morph is not obvious, and was first proved in 
1944 by Cairns~\cite{c-dplc-44} for the case of triangulations.
Cairns used an inductive proof, based on contracting a low-degree vertex to a neighbor.
In general,  a contraction that preserves planarity in both drawings may not exist, so Cairns needed a preliminary morphing procedure to make this possible.  As a result, his method %, although constructive, 
involved two recursive calls, and took an exponential number of steps.
%Thomassen~\cite{t-dpg-83} extended the proof to all straight-line planar graph drawings 
%by augmenting both drawings to isomorphic (``compatible'') triangulations~\cite{ASS}. 
%Thomassen~\cite{t-dpg-83} extended the proof to all straight-line planar graph drawings.  His basic idea was to augment both drawings to triangulations, but this is  
%non-trivial because both augmented drawings must represent the same graph.  
Thomassen~\cite{t-dpg-83} extended the proof to all planar straight-line drawings. He did this by augmenting both drawings to  isomorphic (``compatible'') triangulations which reduces the general case to Cairns's result. The idea of compatible triangulations was rediscovered and thoroughly explored by Aronov et al.~\cite{ASS}, who showed, among other things, that two drawings of a graph on $n$ vertices have a compatible triangulation of size $O(n^2)$ and that this bound is tight in the worst case.
 
%{\smallskip\noindent\bf Continuous Morph.}
Floater and Gotsman~\cite{FG} gave an alternative way to morph straight-line planar triangulations based on Tutte's graph drawing algorithm~\cite{Tutte}.
Gotsman and Surazhsky~\cite{GS,surazhsky-mpt-99,SG,SG2} extended the method to all straight-line planar graph drawings using the same idea of compatible triangulations, and they showed that the resulting morphs are visually appealing.
These algorithms do not produce explicit vertex trajectories; instead, they compute the intermediate drawing (a ``snapshot''') at any requested time point.  There are no quality guarantees about the number of time-points required to approximate continuous motion while preserving planarity.  
%For further discussion of this method see the background section, Section~\ref{sec:background}.
For related results, see~\cite{ekp-ifmpg-03,ekp-mpg-04,fe-gdm-02}.


%{\smallskip\noindent\bf Piece-Wise Linear Morphs.}
%Cairns's method, although exponential, uses discrete steps, whereas the method of Floater and Gotsman does not.
The problem of finding a straight-line planar morph that uses a polynomial number of discrete steps has been asked several times
 (see, e.g.,~\cite{km-mpgss-08,l-mpgd-07,LP,LPS}).  
The most natural definition of a discrete step is a \emph{linear morph}, where every vertex moves along a straight-line segment at uniform speed.  
Note that we do not require that all vertices move at the same speed.
One of the surprising things we discovered (after our first conference version~\cite{SODA-morph}) is that it is actually easier to solve our problem using a more restrictive type of linear morph.  
Specifically, we define a morph to be \emph{unidirectional} if every vertex moves along a straight-line segment at uniform speed, and all the lines of motion are parallel. As a special case, a linear morph that only moves one vertex is unidirectional by default.  
%Our algorithm will sometimes move multiple vertices at once. 
%\rednote{Is there an example to show that we cannot morph by moving one vertex at a time?}

% this will go in definitions:
%A linear morph is completely specified by the initial and final vertex positions.
%If $\Gamma_1$ and $\Gamma_2$ are straight-line planar drawings of a graph, we use $\morph{\Gamma_1, \Gamma_2}$ to denote the linear morph from $\Gamma_1$ to $\Gamma_2$. 
%We seek a morph that consists of a sequence of $k$ linear morphs (a ``piece-wise linear morph'').
%Such a morph can be specified by $k+1$ planar straight-line graph drawings.   If $\Gamma_1, \ldots, \Gamma_{k+1}$ are straight-line planar drawings of a graph, we use $\morph{\Gamma_1, \ldots, \Gamma_{k+1}}$ to denote the morph from $\Gamma_1$ to $\Gamma_{k+1}$ that consists of the $k$ linear morphs from $\Gamma_i$ to $\Gamma_{i+1}$ for $i=1, \ldots, k$.


%{\smallskip\noindent\bf Our Result.}
\subsection{Main Result}
\label{sec:main-result}

The main result of this paper is the following:

\begin{theorem}\label{th:main}
Given a planar graph $G$ on $n$ vertices and two straight-line planar drawings of $G$ with the same faces, the same outer face, and the same nesting of connected components, there is  
a morph between the two drawings that preserves straight-line planarity and consists of \update{$O(n)$ unidirectional morphs}.  Furthermore, the morph can be found in time $O(n^3)$.
%Let $\Gamma_s$ and $\Gamma_t$ be two drawings of the same connected plane graph $G$.
%There exists a morph \mmorph{\Gamma_s,\dots,\Gamma_t} with $O(n^2)$
%steps transforming $\Gamma_s$ into $\Gamma_t$.
\end{theorem}

\update{In addition, we show that $\Omega(n)$ is a lower bound on the number of unidirectional morphs required in the worst case.}

This paper is based on \update{four conference papers: \cite{SODA-morph} for triangulated graphs; 
\cite{Barrera-unidirectional} for unidirectional morphs;
\cite{angelini2013morphing} for non-triangulated graphs;
\cite{Angelini-optimal-14} for achieving a linear number of steps and for the lower bound}.  New to this version is the handling of disconnected graphs.

\remove{
A more recent conference publication~\cite{Angelini-optimal-14} reduces the bound in Theorem~\ref{th:main} to $O(n)$ unidirectional morphs, which is optimal.  
This improvement is achieved via a better algorithm for one subroutine of our algorithm, Quadrilateral Convexification (described in more detail below).
}  

Techniques from our paper have %also 
been used in algorithms to morph Schnyder drawings~\cite{Barrera-Cruz-Schnyder}, and algorithms to morph convex drawings while preserving convexity~\cite{adflpr-omcd-15}. 

\remove{
We note that a newer result~\cite{Angelini-optimal-14} reduces the bound in Theorem~\ref{th:main} to a total of $O(n)$ unidirectional morphs, which is optimal. While this new result supersedes ours, all its main ideas are borrowed from our paper, with the exception of an elegant solution to the Quadrilateral Convexification problem with $O(1)$ unidirectional morphs, achieved via a previously unseen connection between that problem and the existence of hierarchical planar convex drawings of hierarchical planar triconnected graphs. Beside the use of this connection, the algorithm in~\cite{Angelini-optimal-14} is {\em exactly} the same as ours, which justifies our belief that this paper has been foundational to all subsequent research done in this topic (see~\cite{Angelini-optimal-14},~\cite{Barrera-Cruz-Schnyder} for algorithms to morph Schnyder drawings, and~\cite{adflpr-omcd-15} for algorithms to construct convex morphs).
} 



From a high-level perspective, 
our proof of Theorem~\ref{th:main} has two parts: to solve the problem for the special case of a maximal planar graph, in which case both drawings are triangulations; and to reduce the general problem to this special case. 

Previous papers~\cite{SODA-morph,GS,t-dpg-83} reduced the general case to the case of triangulations by finding 
``compatible'' triangulations of both drawings, which increases the size of the graph to $O(n^2)$.
We improve this by making use of the freedom to morph the drawings.  
Specifically, we show that after a sequence of \update{$O(n)$ unidirectional morphs} 
we can triangulate both drawings with the same edges.
% (and with no extra vertices).  -- but there are 3 extra vertices
Thus we reduce the general problem to the case of triangulations with the same input size.



For the case of triangulations, the main idea of our algorithm is the same one that Cairns used to prove existence of a morph, namely to find a vertex $v$ that can be contracted in both drawings to a neighbor $u$ while preserving planarity.
Contracting $v$ to $u$ gives us two planar drawings of a smaller graph.
Using recursion, we can find a morph between the smaller drawings that consists of unidirectional morphs.
Thus the total process is to move $v$ along a straight line to $u$ in the first drawing (a unidirectional morph since only one vertex moves), perform the recursively computed morph, and then, in the second drawing, reverse the motion of $v$ to $u$.  

Note that this process allows a vertex to become coincident with another vertex, so it is not a true morph, but rather what we call a  ``pseudomorph''. 
There are two main issues with this plan: 
 (1) to deal with the fact that  there may not be a vertex $v$ that can be contracted to the same neighbor $u$ in both drawings; and 
(2) to convert a pseudomorph to a morph. 
We will give a few more details on each of these.

A contractible vertex always exists if we are dealing with a single triangulation:
because the graph is planar, there is an internal vertex  $v$ of degree less than or equal to 5; because the graph is triangulated, the neighbors of $v$ form a polygon of at most 5 vertices; and by an easy geometric argument, such a polygon always has a vertex $u$ that ``sees'' the whole polygon, so $v$ can be contracted to $u$ while preserving planarity.  
%\rednote{AL. Maybe make a figure.}
In our situation there is one complication---we want to contract $v$ to the same neighbor in both drawings.
This is easy to solve in the case where our low-degree vertex $v$ has neighbors that form a convex polygon in the first drawing---in this case every neighbor of $v$ sees the whole convex polygon in the first drawing, so we can choose the vertex $u$ that works in the second drawing.  Our general solution will be to morph the first drawing so that $v$'s neighbors form a convex polygon (or at least ``convex enough'' in the sense that $u$ sees the whole polygon).   This was the same approach that Cairns used, though his solution required an exponential number of morphing steps, and our solution will be efficient.

To summarize the first part of our algorithm to morph between two triangulations: we show that after \update{$O(1)$ unidirectional morphs} we can obtain a vertex $v$ that can be contracted to the same neighbor in both drawings. 

After performing the contraction we apply induction to find a morph (composed of unidirectional morphs) between the two smaller drawings.  
The last issue is to convert the resulting pseudomorph to a true morph.
Instead of contracting $v$ to a neighbor $u$, we must keep $v$ close to, but not coincident with, $u$, while we follow the morph of the smaller graph. 
Cairns solved this issue by keeping $v$ at the centroid of its surrounding polygon, but this results in %a
non-linear motion for $v$.
We will find a position for $v$ in each drawing during the course of the morph so that the linear motion from one drawing to the next remains unidirectional.

Putting together the two parts of our algorithm, the total number of unidirectional morphs satisfies \update{$S(n) = S(n-1) + O(1)$ which solves to $O(n)$}.  

This completes the high-level overview of our algorithm.  From a low-level perspective, the 
heart of our algorithm is a solution to a problem we call \emph{Quadrilateral Convexification}: given a triangulation and a non-convex quadrilateral in the drawing, morph the triangulation to make the quadrilateral convex.  
%\rednote{AL: Refer to a figure?}


Our morphing algorithm uses $O(n)$ calls to Quadrilateral Convexification, plus $O(n)$ other unidirectional morphs.  We will show that Quadrilateral Convexification
can be solved with \update{$O(1)$ unidirectional morphs}.   Thus our total bound is \update{$O(n)$ unidirectional morphs}. 
\update{
Our original conference version of this result~\cite{SODA-morph} required $O(n)$ linear morphs for each Quadrilateral Convexification via a recursive solution (contracting a low degree vertex to a neighbor).  Here we present an improvement to $O(1)$ unidirectional morphs first presented in~\cite{Angelini-optimal-14}. 
The improvement is achieved via a previously unseen connection to the existence of hierarchical planar convex drawings of hierarchical planar triconnected graphs which will be presented in Section~\ref{sec:quad-convexification}.
}

\remove{
As noted above, a newer result~\cite{Angelini-optimal-14} solves Quadrilateral Convexification with $O(1)$ unidirectional morphs, thus reducing the bound in our main result to a total of $O(n)$ unidirectional morphs.  
The improvement in Quadrilateral Convexification is achieved via a previously unseen connection to the existence of hierarchical planar convex drawings of hierarchical planar triconnected graphs.
}

\update{We also prove that our linear bound is optimal---more precisely, that straightening an $n$-vertex spiral requires $\Omega(n)$ linear morphing steps.}

The rest of the paper is organized as follows. First, in
Section~\ref{sec:definitions} we give formal definitions of our terms and concepts.
Then in Section~\ref{se:overview} we give a more detailed outline of the algorithm.  We fill in solutions to the various subproblems in the following sections. 
\update{Finally, the lower bound is in Section~\ref{sec:lower-bound}.}


\remove{  % Everything here is covered elsewhere except the refs. \cite{ACDP}, \cite{BLS-orth}, \cite{Spriggs}
\subsection{Further Background}
\label{sec:background}

\rednote{AL. This section is still disorganized, but I will fix it.}
A result by Angelini et al.~\cite{ACDP} addresses the problem of ``topological morphing'' where the planar embedding changes.  However most work, including ours,  is about the case where the initial and final planar drawings are \emph{topologically equivalent}---i.e., have the same faces and the same outer face---and planarity must be preserved throughout the morph.

We note that Thomassen~\cite{t-dpg-83} also showed that there exists a morph that preserves convexity in addition to straight-line planarity.

The case of preserving more general edge directions is explored in~\cite{BLS-orth}
%by  Biedl et al.~\cite{BLS-orth} 
and in the thesis of Spriggs~\cite{Spriggs}.


An alternative approach to morphing planar straight-line triangulations was presented by Floater and Gotsman~\cite{FG}.  Their method is based on Tutte's graph drawing algorithm~\cite{Tutte}, in which the position of each vertex is expressed as a convex combination of the positions of its neighbors.  Any matrix of such coefficients provides a planar drawing. So Floater and Gotsman
expressed each of the given drawings by means of a matrix of coefficients, and then took a linear interpolation between the matrices to obtain the morph.
Gotsman and Surazhsky~\cite{GS,surazhsky-mpt-99,SG,SG2} extended the method to all planar straight-line graph drawings, and showed that the resulting morphs are visually appealing.
The algorithm does not produce explicit vertex trajectories.  It computes, at any given time-point of the morph, a ``snapshot'' of the graph at that time.  In other words, it provides an efficient implementation of a black-box representation of the morph, where an input time-point is mapped to an output graph drawing.
There are no quality guarantees about the number of time-points required to approximate continuous motion, or about the grid size of the drawings or the minimum feature size (the measure of how close a vertex and non-incident edge may be).
For related results, see~\cite{ekp-ifmpg-03,ekp-mpg-04,fe-gdm-02}.

\rednote{AL. Also mention Schnyder morphing.}
}



==> introduction.tex <==
\section{Introduction}\label{se:intro}

A morph between two geometric shapes is a continuous transformation of one shape into
the other. 
Morphs are useful in many areas of computer science---Computer Graphics, Animation, and Modeling, to name just a few.
%Computer Graphics, Animation, and Modeling are only few of the areas of Computer Science that make use of morphs.
The usual goal in morphing is to ensure that the structure of the shapes be ``visible'' throughout the entire transformation.

%Graph drawing has developed into a mature field with a rich mix of applications and theory.
%See the books~\cite{DETT,Kaufmann-Wagner} and the forthcoming handbook~\cite{handbook}.
%Recently, several papers have addressed the problem of \emph{morphing} graph drawings. 


Two-dimensional graph drawings can be used to represent many of the shapes for which morphs are of interest, e.g., two-dimensional
images~\cite{bn-fbim-92,fm-ffip-98,te-imfpt-99}, polygons, and  poly-lines~\cite{aadddhlrssw-cpwlv-11,acl-arpsi-00,cc-wgosm-97,elrsw-cssp-98,gh-msp-94,nmwb-mpstcg-08,sgwm-2dsbisvpp-93,sg-pba2dsb-92,sr-sbussr-95}. 
For this reason, morphs of graph drawings have been well studied. 

For the problem of morphing graph drawings,  
%In this context, 
the input consists of two 
drawings $\Gamma_1$ and $\Gamma_2$ of the same graph $G$, and the problem is to transform continuously from the first drawing to the second drawing.
%one drawing to the other. 
A \emph{morph} between $\Gamma_1$ and $\Gamma_2$ is  a continuously changing family of drawings of $G$ indexed by time $t \in  [0, 1]$, such that the drawing at time $t = 0$ is $\Gamma_1$ and the drawing at time $t = 1$ is $\Gamma_2$. 
%Preserving 
Maintaining structure during the morph becomes a matter of preserving geometric properties such as planarity, straight-line planarity, edge lengths, or edge directions.
For example, preserving edge lengths in a straight-line drawing leads to problems of linkage reconfiguration~\cite{CDR,DO'R}.

%{\smallskip\noindent\bf Morphing Planar Graph Drawings.}
In this paper we consider the problem of morphing between two graph drawings while preserving planarity.
Of necessity, we 
assume that the initial and final planar drawings are \emph{topologically equivalent}---i.e., have the same faces and the same outer face.
In addition to the above-mentioned applications, morphing graph drawings while preserving planarity has application to the problem of creating three-dimensional models from two-dimensional slices~\cite{BS}, with time playing the role of the third dimension.

When planar graphs may be drawn with poly-line edges the morphing problem becomes much easier---the intuition is that vertices can move around while edges bend to avoid collisions.  An efficient morphing algorithm for this case was given by 
Lubiw and Petrick~\cite{LP}. 
The case of orthogonal graph drawings is also well-solved---Biedl et al.~\cite{biedl2013morphing} gave
%a SODA'06 paper describes 
an algorithm to morph efficiently between any two orthogonal drawings of the same graph while preserving planarity and orthogonality.

%{\smallskip\noindent\bf Morphing Straight-Line Planar Drawings.}
We restrict our attention in this paper to straight-line planar drawings.
Our main result is an efficient algorithm to morph between two topologically equivalent straight-line planar drawings of a graph, where the morph must preserve straight-line planarity.  The issue is to find the vertex trajectories, since the edges are determined by the vertex positions.

%{\smallskip\noindent\bf Existence.}
Existence of such a morph is not obvious, and was first proved in 
1944 by Cairns~\cite{c-dplc-44} for the case of triangulations.
Cairns used an inductive proof, based on contracting a low-degree vertex to a neighbor.
In general,  a contraction that preserves planarity in both drawings may not exist, so Cairns needed a preliminary morphing procedure to make this possible.  As a result, his method %, although constructive, 
involved two recursive calls, and took an exponential number of steps.
%Thomassen~\cite{t-dpg-83} extended the proof to all straight-line planar graph drawings 
%by augmenting both drawings to isomorphic (``compatible'') triangulations~\cite{ASS}. 
%Thomassen~\cite{t-dpg-83} extended the proof to all straight-line planar graph drawings.  His basic idea was to augment both drawings to triangulations, but this is  
%non-trivial because both augmented drawings must represent the same graph.  
Thomassen~\cite{t-dpg-83} extended the proof to all planar straight-line drawings. He did this by augmenting both drawings to  isomorphic (``compatible'') triangulations which reduces the general case to Cairns's result. The idea of compatible triangulations was rediscovered and thoroughly explored by Aronov et al.~\cite{ASS}, who showed, among other things, that two drawings of a graph on $n$ vertices have a compatible triangulation of size $O(n^2)$ and that this bound is tight in the worst case.
 
%{\smallskip\noindent\bf Continuous Morph.}
Floater and Gotsman~\cite{FG} gave an alternative way to morph straight-line planar triangulations based on Tutte's graph drawing algorithm~\cite{Tutte}.
Gotsman and Surazhsky~\cite{GS,surazhsky-mpt-99,SG,SG2} extended the method to all straight-line planar graph drawings using the same idea of compatible triangulations, and they showed that the resulting morphs are visually appealing.
These algorithms do not produce explicit vertex trajectories; instead, they compute the intermediate drawing (a ``snapshot''') at any requested time point.  There are no quality guarantees about the number of time-points required to approximate continuous motion while preserving planarity.  
%For further discussion of this method see the background section, Section~\ref{sec:background}.
For related results, see~\cite{ekp-ifmpg-03,ekp-mpg-04,fe-gdm-02}.


%{\smallskip\noindent\bf Piece-Wise Linear Morphs.}
%Cairns's method, although exponential, uses discrete steps, whereas the method of Floater and Gotsman does not.
The problem of finding a straight-line planar morph that uses a polynomial number of discrete steps has been asked several times
 (see, e.g.,~\cite{km-mpgss-08,l-mpgd-07,LP,LPS}).  
The most natural definition of a discrete step is a \emph{linear morph}, where every vertex moves along a straight-line segment at uniform speed.  
Note that we do not require that all vertices move at the same speed.
One of the surprising things we discovered (after our first conference version~\cite{SODA-morph}) is that it is actually easier to solve our problem using a more restrictive type of linear morph.  
Specifically, we define a morph to be \emph{unidirectional} if every vertex moves along a straight-line segment at uniform speed, and all the lines of motion are parallel. As a special case, a linear morph that only moves one vertex is unidirectional by default.  
%Our algorithm will sometimes move multiple vertices at once. 
%\rednote{Is there an example to show that we cannot morph by moving one vertex at a time?}

% this will go in definitions:
%A linear morph is completely specified by the initial and final vertex positions.
%If $\Gamma_1$ and $\Gamma_2$ are straight-line planar drawings of a graph, we use $\morph{\Gamma_1, \Gamma_2}$ to denote the linear morph from $\Gamma_1$ to $\Gamma_2$. 
%We seek a morph that consists of a sequence of $k$ linear morphs (a ``piece-wise linear morph'').
%Such a morph can be specified by $k+1$ planar straight-line graph drawings.   If $\Gamma_1, \ldots, \Gamma_{k+1}$ are straight-line planar drawings of a graph, we use $\morph{\Gamma_1, \ldots, \Gamma_{k+1}}$ to denote the morph from $\Gamma_1$ to $\Gamma_{k+1}$ that consists of the $k$ linear morphs from $\Gamma_i$ to $\Gamma_{i+1}$ for $i=1, \ldots, k$.


%{\smallskip\noindent\bf Our Result.}
\subsection{Main Result}
\label{sec:main-result}

The main result of this paper is the following:

\begin{theorem}\label{th:main}
Given a planar graph $G$ on $n$ vertices and two straight-line planar drawings of $G$ with the same faces, the same outer face, and the same nesting of connected components, there is  
a morph between the two drawings that preserves straight-line planarity and consists of $O(n^2)$ unidirectional morphs.  Furthermore, the morph can be found in time $O(n^3)$.
%Let $\Gamma_s$ and $\Gamma_t$ be two drawings of the same connected plane graph $G$.
%There exists a morph \mmorph{\Gamma_s,\dots,\Gamma_t} with $O(n^2)$
%steps transforming $\Gamma_s$ into $\Gamma_t$.
\end{theorem}

This paper is based on three conference papers: \cite{SODA-morph} for triangulated graphs; 
\cite{Barrera-unidirectional} for unidirectional morphs;
\cite{angelini2013morphing} for non-triangulated graphs.  New to this version is the handling of disconnected graphs.

A more recent conference publication~\cite{Angelini-optimal-14} reduces the bound in Theorem~\ref{th:main} to $O(n)$ unidirectional morphs, which is optimal.  
This improvement is achieved via a better algorithm for one subroutine of our algorithm, Quadrilateral Convexification (described in more detail below).  Techniques from our paper have also been used in algorithms to morph Schnyder drawings~\cite{Barrera-Cruz-Schnyder}, and algorithms to morph convex drawings while preserving convexity~\cite{adflpr-omcd-15}. 

\remove{
We note that a newer result~\cite{Angelini-optimal-14} reduces the bound in Theorem~\ref{th:main} to a total of $O(n)$ unidirectional morphs, which is optimal. While this new result supersedes ours, all its main ideas are borrowed from our paper, with the exception of an elegant solution to the Quadrilateral Convexification problem with $O(1)$ unidirectional morphs, achieved via a previously unseen connection between that problem and the existence of hierarchical planar convex drawings of hierarchical planar triconnected graphs. Beside the use of this connection, the algorithm in~\cite{Angelini-optimal-14} is {\em exactly} the same as ours, which justifies our belief that this paper has been foundational to all subsequent research done in this topic (see~\cite{Angelini-optimal-14},~\cite{Barrera-Cruz-Schnyder} for algorithms to morph Schnyder drawings, and~\cite{adflpr-omcd-15} for algorithms to construct convex morphs).
} 



From a high-level perspective, 
our proof of Theorem~\ref{th:main} has two parts: to solve the problem for the special case of a maximal planar graph, in which case both drawings are triangulations; and to reduce the general problem to this special case. 

Previous papers~\cite{SODA-morph,GS,t-dpg-83} reduced the general case to the case of triangulations by finding 
``compatible'' triangulations of both drawings, which increases the size of the graph to $O(n^2)$.
We improve this by making use of the freedom to morph the drawings.  
Specifically, we show that after a sequence of $O(n^2)$ unidirectional morphs 
we can triangulate both drawings with the same edges.
% (and with no extra vertices).  -- but there are 3 extra vertices
Thus we reduce the general problem to the case of triangulations with the same input size.



For the case of triangulations, the main idea of our algorithm is the same one that Cairns used to prove existence of a morph, namely to find a vertex $v$ that can be contracted in both drawings to a neighbor $u$ while preserving planarity.
Contracting $v$ to $u$ gives us two planar drawings of a smaller graph.
Using recursion, we can find a morph between the smaller drawings that consists of unidirectional morphs.
Thus the total process is to move $v$ along a straight line to $u$ in the first drawing (a unidirectional morph since only one vertex moves), perform the recursively computed morph, and then, in the second drawing, reverse the motion of $v$ to $u$.  

Note that this process allows a vertex to become coincident with another vertex, so it is not a true morph, but rather what we call a  ``pseudomorph''. 
There are two main issues with this plan: 
 (1) to deal with the fact that  there may not be a vertex $v$ that can be contracted to the same neighbor $u$ in both drawings; and 
(2) to convert a pseudomorph to a morph. 
We will give a few more details on each of these.

A contractible vertex always exists if we are dealing with a single triangulation:
because the graph is planar, there is an internal vertex  $v$ of degree less than or equal to 5; because the graph is triangulated, the neighbors of $v$ form a polygon of at most 5 vertices; and by an easy geometric argument, such a polygon always has a vertex $u$ that ``sees'' the whole polygon, so $v$ can be contracted to $u$ while preserving planarity.  
%\rednote{AL. Maybe make a figure.}
In our situation there is one complication---we want to contract $v$ to the same neighbor in both drawings.
This is easy to solve in the case where our low-degree vertex $v$ has neighbors that form a convex polygon in the first drawing---in this case every neighbor of $v$ sees the whole convex polygon in the first drawing, so we can choose the vertex $u$ that works in the second drawing.  Our general solution will be to morph the first drawing so that $v$'s neighbors form a convex polygon (or at least ``convex enough'' in the sense that $u$ sees the whole polygon).   This was the same approach that Cairns used, though his solution required an exponential number of morphing steps, and our solution will be efficient.

To summarize the first part of our algorithm to morph between two triangulations: we show that after $O(n)$ unidirectional morphs we can obtain a vertex $v$ that can be contracted to the same neighbor in both drawings. 

After performing the contraction we apply induction to find a morph (composed of unidirectional morphs) between the two smaller drawings.  
The last issue is to convert the resulting pseudomorph to a true morph.
Instead of contracting $v$ to a neighbor $u$, we must keep $v$ close to, but not coincident with, $u$, while we follow the morph of the smaller graph. 
Cairns solved this issue by keeping $v$ at the centroid of its surrounding polygon, but this results in %a
non-linear motion for $v$.
We will find a position for $v$ in each drawing during the course of the morph so that the linear motion from one drawing to the next remains unidirectional.

Putting together the two parts of our algorithm, the total number of unidirectional morphs satisfies $S(n) = S(n-1) + O(n)$ which solves to $O(n^2)$.  

This completes the high-level overview of our algorithm.  From a low-level perspective, the 
heart of our algorithm is a solution to a problem we call \emph{Quadrilateral Convexification}: given a triangulation and a non-convex quadrilateral in the drawing, morph the triangulation to make the quadrilateral convex.  
%\rednote{AL: Refer to a figure?}


Our morphing algorithm uses $O(n)$ calls to Quadrilateral Convexification, plus $O(n)$ other unidirectional morphs.  We will show that Quadrilateral Convexification
can be solved with $O(n)$ unidirectional morphs.   Thus our total bound is $O(n^2)$ unidirectional morphs. 

As noted above, a newer result~\cite{Angelini-optimal-14} solves Quadrilateral Convexification with $O(1)$ unidirectional morphs, thus reducing the bound in our main result to a total of $O(n)$ unidirectional morphs.  
The improvement in Quadrilateral Convexification is achieved via a previously unseen connection to the existence of hierarchical planar convex drawings of hierarchical planar triconnected graphs.

The rest of the paper is organized as follows. First, in
Section~\ref{sec:definitions} we give formal definitions of our terms and concepts.
Then in Section~\ref{se:overview} we give a more detailed outline of the algorithm.  We fill in solutions to the various subproblems in the following sections. 


\remove{  % Everything here is covered elsewhere except the refs. \cite{ACDP}, \cite{BLS-orth}, \cite{Spriggs}
\subsection{Further Background}
\label{sec:background}

\rednote{AL. This section is still disorganized, but I will fix it.}
A result by Angelini et al.~\cite{ACDP} addresses the problem of ``topological morphing'' where the planar embedding changes.  However most work, including ours,  is about the case where the initial and final planar drawings are \emph{topologically equivalent}---i.e., have the same faces and the same outer face---and planarity must be preserved throughout the morph.

We note that Thomassen~\cite{t-dpg-83} also showed that there exists a morph that preserves convexity in addition to straight-line planarity.

The case of preserving more general edge directions is explored in~\cite{BLS-orth}
%by  Biedl et al.~\cite{BLS-orth} 
and in the thesis of Spriggs~\cite{Spriggs}.


An alternative approach to morphing planar straight-line triangulations was presented by Floater and Gotsman~\cite{FG}.  Their method is based on Tutte's graph drawing algorithm~\cite{Tutte}, in which the position of each vertex is expressed as a convex combination of the positions of its neighbors.  Any matrix of such coefficients provides a planar drawing. So Floater and Gotsman
expressed each of the given drawings by means of a matrix of coefficients, and then took a linear interpolation between the matrices to obtain the morph.
Gotsman and Surazhsky~\cite{GS,surazhsky-mpt-99,SG,SG2} extended the method to all planar straight-line graph drawings, and showed that the resulting morphs are visually appealing.
The algorithm does not produce explicit vertex trajectories.  It computes, at any given time-point of the morph, a ``snapshot'' of the graph at that time.  In other words, it provides an efficient implementation of a black-box representation of the morph, where an input time-point is mapped to an output graph drawing.
There are no quality guarantees about the number of time-points required to approximate continuous motion, or about the grid size of the drawings or the minimum feature size (the measure of how close a vertex and non-incident edge may be).
For related results, see~\cite{ekp-ifmpg-03,ekp-mpg-04,fe-gdm-02}.

\rednote{AL. Also mention Schnyder morphing.}
}



==> makefile <==
finalname = journal
compiler = xelatex
bibcomp = bibtex

included_latex_sources = 

psfiles = \


$(finalname): $(included_latex_sources) $(psfiles) $(finalname).tex
	$(compiler) $(finalname).tex

%.ps: %.fig
	fig2dev -Leps $< $@

%.ps: %.gif
	convert $< $@

%.ps: %.bmp
	convert $< $@

%.ps: %.jpg
	convert $< $@

startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.pdf
	rm -f *.out
	rm -f *.bbl
	rm -f *.dep

bib: 
	$(compiler) $(finalname).tex
	$(bibcomp) $(finalname)
	$(compiler) $(finalname).tex
	$(compiler) $(finalname).tex


ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o

pdf: $(finalname)
#	dvips -Ppdf $(finalname).dvi -o $(finalname).ps
#	ps2pdf $(finalname).ps $(finalname).pdf
	pdflatex $(finalname)

print: ps
	lpr -Ppolaris -h $(finalname).ps

bundle:	clean bib
	bundledoc --verbose --include="*.bib" --include="makefile" --exclude="MANIFEST" $(finalname).dep


==> packages.tex <==
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
% \usepackage{ntheorem}
\usepackage{mathtools}

\usepackage{graphicx}
%\usepackage{subfig}
% \usepackage{epsfig}

\usepackage{xspace}
\usepackage{paralist} % package for inline lists
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage[pdfborder={0.5 0.5 0.5}]{hyperref}
\usepackage[figure]{hypcap}
\usepackage{subfigure}
%\usepackage{subfig}

%\usepackage{cleveref}
%\usepackage{ltexpprt}

\usepackage[english]{babel}
% \usepackage[latin1]{inputenc} 
\usepackage[T1]{fontenc}
\usepackage{tikz}
\usetikzlibrary{arrows,calc,decorations.text}

\usepackage{todonotes}

\usepackage[plain,ruled]{algorithm}
\usepackage[noend]{algorithmic}

\usepackage{fullpage}
\usepackage{lineno}



==> quad-convexification.tex <==
\section{Quadrilateral Convexification}
\label{sec:quad-convexification}

In this section we give an algorithm for Problem~\ref{prob:quad-convex}, to convexify a quadrilateral by means of a morph composed of unidirectional morphing steps.  
The main result of the section is as follows:

%\begin{theorem*}{\bf [Reminder of Theorem~\ref{thm:quad-convex}.]}
%\quadconvex
%\end{theorem*}
\rephrase{Reminder of Theorem~\ref{thm:quad-convex}}{\quadconvex}

In the rest of this section we will prove the theorem.
Recall that we have 
 an $n$-vertex triangulation $\Gamma$ with triangular outer boundary and a quadrilateral $abcd$ in $\Gamma$ with no vertex inside it  and such that neither $ac$ nor $bd$ is an edge outside of $abcd$.
 Our goal is to  
morph $\Gamma$ so that $abcd$ becomes convex while the outer boundary remains fixed.

Suppose the triangular outer boundary of the drawing is $z_1z_2z_3$.  
If $abcd$ is convex, we are done. Assume without loss of generality that $d$ is the reflex vertex of the non-convex quadrilateral, and thus $b$ is the tip of the arrowhead shape  (see Figure~\ref{fig:4-gon}).
The triangulation contains the edge $bd$.

\begin{figure}[h]
\label{fig:4-gon}
\centering
\includegraphics[width=1.2in]{fig/4-gon.pdf}
\caption{A non-convex quadrilateral $abcd$.}
\end{figure}

We follow Cairns's idea of reducing the size of the problem by one by contracting a non-boundary vertex $v$ with $\Deg(v)\le5$ to a neighbor, recursively solving the problem on the smaller graph, and then uncontracting $v$.
We will find a pseudomorph whose morphing steps are unidirectional and rely on Theorem~\ref{thm:pseudomorph} to convert the pseudomorph to a morph with the same number of unidirectional morphing steps.

A planar graph always has a vertex $v$ of degree at most 5, but not all such vertices are useful for our purposes.
In particular, we must keep the outer boundary fixed,  
we must not ``destroy'' quadrilateral $abcd$, and we must not introduce the edge $ac$ when we contract $v$, since the external chord $ac$ would preclude convexification of $abcd$. 
%We will distinguish the \emph{non-problematic} vertices whose contraction preserves the properties we need.  More precisely, 
Formally, we define a vertex $v$ to be \emph{problematic} if:
\begin{itemize}
  \item  $v$ is a boundary vertex (one of $z_1,z_2,z_3$),
  \item $v$ is a quadrilateral vertex (one of $a,b,c,d$), or
  \item $v$ is $ac$-\emph{inducing}, that is, $v$ has degree at most 5, $v$ is not a boundary or quadrilateral vertex, $v$ is adjacent to both $a$ and $c$, and $v$ is $a$-contractible or $c$-contractible.  
  (We use the term ``$ac$-inducing'' because contracting $v$ to $a$ or $c$ would introduce edge $ac$.)
\end{itemize}

If there is a non-problematic vertex $v$ of degree at most 5 then we contract $v$ to a neighbor, recursively solve the quadrilateral convexification problem in the smaller graph, and then uncontract $v$.  
By Theorem~\ref{thm:pseudomorph} we can convert this pseudomorph to a morph with the same number of unidirectional morphing steps. 
The total number of unidirectional morphing steps then satisfies $S(n) = S(n-1) + O(1)$, which solves to $S(n) \in O(n)$. 

It remains to deal with the case where all vertices of degree at most 5 are problematic.  
We will show that we can find a constant number of unidirectional morphing steps that either convexify the quadrilateral $abcd$ or reduce the problem size.  

Formally, we say that a triangulation is \emph{accommodating} if we have one of the following:
\begin{enumerate}
\item a non-problematic vertex of degree at most 5,
\item a vertex of the quadrilateral that is not on the boundary and has degree at most 4, 
\item a boundary vertex of degree 3 or three boundary vertices of degree 4, or
\item more than one $ac$-inducing vertex.
\end{enumerate}

In the subsections below we show how to handle each of the accommodating situations.  (We already know how to handle the first situation.) 
Theorem~\ref{thm:quad-convex} then follows from a counting argument that shows that every triangulation is accommodating:

\begin{lemma} Every triangulation is accommodating.
\label{lem:accommodating}
\end{lemma}
\begin{proof}
Define the \emph{value} of a vertex $v$ to be $6 - \Deg(v)$.  Because the number of edges in a triangulation is $3n-6$, the total value of all vertices is $6n - \sum_v \Deg(v) = 12$.

Suppose the triangulation is not accommodating. Then the three boundary vertices have degrees at least $4$, $4$, and $5$, i.e.~total value at most $5$.  
Any vertex of the quadrilateral that is not on the boundary has degree at least $5$, so the total value of the quadrilateral non-boundary vertices is at most $4$.  There can be at most one $ac$-inducing vertex $v$, and it cannot have degree 3 otherwise its 3 neighbors would be connected, and therefore $ac$ would be an edge, violating our assumption.  This implies that the total value of $ac$-inducing vertices is at most 2. 
All other vertices have degree at least 6, hence value at most 0.  
Thus, the total value of all vertices is at most 11, a contradiction.
\end{proof}


We now discuss the running time of the algorithm to compute the morph for Quadrilateral Convexification.  
At each step we find a vertex to contract, recursively find a morph of the smaller graph, and then appeal to Theorem~\ref{thm:pseudomorph} to convert the resulting pseudomorph to a morph with the same number of unidirectional morphing steps.  The number of unidirectional morphs is always $O(n)$.  Each time we convert a pseudomorph to a morph, this takes $O(n)$ time (by Theorem~\ref{thm:pseudomorph}).  Thus, the time spent on pseudomorph conversion alone is $T(n) = T(n-1) + O(n)$, which solves to $T(n) \in O(n^2)$.  
We also need to find the vertex to contract or the accommodating situation, and decide how to handle it (with details below).  It is easy to see that in each step this can be accomplished in $O(n)$ time.
%In fact this can probably be reduced to $O(n)$ in total, though such a reduction is irrelevant to the total time bound.
Thus the total running time is $O(n^2)$. 

  
\remove{
As for the work to find the morph, we order the vertices by degree.  We can update this order in constant time per contraction, since we only contract vertices of degree at most 5.
We perform a linear search through the vertices of degree at most 5. 
We can test in constant time if a vertex is problematic.  There are at most 8 problematic vertices: 4 quadrilateral vertices, 3 boundary vertices, and (by Lemma~\ref{}) at most 1 $ac$-inducing vertex.
We can test in constant time if we have an accommodating situation.   
In the subsections below, we show that  each accommodating situation can be dealt with in constant time.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Handling Quadrilateral Vertices}

In this subsection we handle the second accommodating situation, namely when there is a vertex of the quadrilateral that is not on the boundary and has degree at most 4.  We will show that we can convexify $abcd$ or reduce the problem size by one by moving one vertex in a straight line, which is a unidirectional morph.

We consider the vertices of the quadrilateral in turn.
Suppose vertex $a$ has degree at most 4 and is not a boundary vertex.  
See Figure~\ref{fig:problematic-quad-a}.
%
\begin{figure}[htb]
\centering
\def\sf{1.4}
\hfill\subfigure[]{\includegraphics[scale=\sf]{fig/problematic-quad-a.pdf}\label{fig:problematic-quad-a}}\hfill
\subfigure[]{\includegraphics[scale=\sf]{fig/problematic-quad-b.pdf}\label{fig:problematic-quad-b}}\hfill
\caption{\subref{fig:problematic-quad-a} Handling vertex $a$. 
\subref{fig:problematic-quad-b}~Handling vertex $b$. 
}
\end{figure}
%
\remove{
\begin{figure}[h]
  \centering
\includegraphics[width=1.5in]{fig/problematic-quad-a.pdf}
  \caption{Handling vertex $a$. }
  \label{fig:problematic-quad-a}
\end{figure}
}
Observe the following fact: in any triangle or quadrilateral, every edge must be incident to at least one vertex that lies in the kernel. Applying this fact to $\Delta(a)$ shows that $b$ or $d$ must be in the kernel of $\Delta(a)$.  
We can thus move $a$ to within a small distance from whichever vertex is in the kernel to directly convexify $abcd$.


The case when vertex $c$ has degree at most 4 and is not a boundary vertex is symmetric.

Next suppose that $b$ has degree at most 4 and is not a boundary vertex. 
See Figure~\ref{fig:problematic-quad-b}.
Then $b$ must have exactly one neighbor $x$ that is not on $abcd$, and $x$ must be adjacent to both $a$ and $c$.  Since $d$ is a reflex vertex of the quadrilateral $\Delta(b)=axcd$, vertex $x$ must be in the kernel of $\Delta(b)$.  So we contract $b$ to $x$, recursively convexify $axcd$, and uncontract $b$.

\remove{
\begin{figure}[h]
  \centering
\includegraphics[width=1.5in]{fig/problematic-quad-b.pdf}
  \caption{Handling vertex $b$.}
  \label{fig:problematic-quad-b}
\end{figure}
}


Finally, suppose that $d$ has degree at most 4 and is not a boundary vertex.
See Figure~\ref{fig:problematic-quad-d}~(a) and~(b).
Note that $d$ cannot have degree 3 because $ac$ is not an edge.  
Thus $d$ must have exactly one neighbor $x$ that is not on $abcd$ and $x$ must be adjacent to $a$ and $c$. 
If $x$ is outside the triangle $abc$ then $a$ and $c$ are in the kernel of $\Delta(d)$, so we can directly convexify $abcd$ by moving $d$ to within a small distance from $a$.
Otherwise we contract $d$ to $x$, recursively convexify $abcx$, and uncontract $d$. 


\begin{figure}[h]
  \centering
\includegraphics[width=3in]{fig/problematic-quad-d.pdf}
  \caption{Handling vertex $d$.}
  \label{fig:problematic-quad-d}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Handling Boundary Vertices}

In this subsection we handle the third accommodating situation, namely when there is a boundary vertex of degree 3 or three boundary vertices of degree 4.
We will show that a single unidirectional morph suffices to convexify $abcd$ or reduce the problem size.


In all the cases so far, we moved one vertex at a time.
To handle boundary vertices we will move one vertex of a triangle along a straight line and have the vertices inside the triangle follow along linearly. By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph.

Suppose boundary vertex $z_1$ has degree 3. 
See Figure~\ref{fig:4-gon-deg-3}~(a).
\begin{figure}[h]
\label{fig:4-gon-deg-3}
\centering
\includegraphics[width=4.5in]{fig/4-gon-deg-3.pdf}
\caption{Handling a boundary vertex of degree 3.}
\end{figure}

Then $z_1$ must have a neighbor $y$ that is adjacent to $z_2$ and $z_3$.  If $abcd$ lies entirely inside the triangle $T=yz_2z_3$ then we recursively morph the subgraph contained in $T$.  Otherwise $abcd$ must include at least one triangle outside $T$.  It cannot have both its triangles outside $T$ by the assumption that there is no edge $ac$.  Thus we can assume without loss of generality that $abcd$ consists of triangle $z_1yz_3$ and an adjacent triangle formed by $z_3 y$ and an internal vertex of $T$, see Figure~\ref{fig:4-gon-deg-3}(b).  
%The solution is to move $y$ towards $z_1$ to directly convexify $abcd$.  As $y$ is moved, the contents of triangle $T$ follow along linearly.  By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph. 
The solution is to move $y$ towards an interior point of the edge $z_1 z_2$ to directly convexify the quadrilateral.  As $y$ is moved, the contents of triangle $T$ follow along linearly.  By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph.   Note that this motion will convexify the quadrilateral since every interior point of $T$ is a convex combination of $y$, $z_2$, and $z_3$ with a positive contribution from $z_3$.

Now suppose that all three boundary vertices have degree 4.  See Figure~\ref{fig:4-gon-deg-4}(a).
In this case there exists an internal triangle $T= y_1 y_2 y_3$ containing all the internal vertices with 
$y_i$ adjacent to $z_j$ for $j \ne i$ with $i,j \in \{1,2,3\}$. 
\begin{figure}[h]
\centering
\includegraphics[width=4.5in]{fig/4-gon-deg-4.pdf}
\caption{Handling the case of three boundary vertices of degree 4.}
\label{fig:4-gon-deg-4}
\end{figure}
%$y_1$ adjacent to $z_2, z_3$ and $y_2$ adjacent to $z_3,z_1$ and $y_3$ adjacent to $z_1, z_2$.   
If $abcd$ lies entirely inside $T$ then we recursively morph the subgraph contained in $T$.  If $abcd$ lies entirely outside $T$ then without loss of generality $abcd$ is $z_1y_3y_2z_3$. The solution is to move $y_3$ towards $z_1$ to directly convexify the
quadrilateral. As $y_3$ is moved, the contents of triangle $T$ follow along linearly.
\remove{  -- Fabrizio's change is below, but I think it belongs with the previous case.  A.L.
The solution is to move $y_3$ 
towards an interior point of edge $z_1 z_3$ to directly convexify the quadrilateral.
%to within a small distance of $z_1$ and perturb it to directly convexify the 4-gon.  
As $y_3$ is moved, the contents of triangle $T$  follow along linearly.  By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph. Note that, if $y_3$ moves sufficiently close to edge $z_1 z_3$, quadrilateral $abcd$ does become convex. Indeed, if $y_3$ moved {\em on} an interior point of edge $z_1 z_3$, then the angle of $abcd$ incident to $y$ would be convex, since the vertex of $abcd$ different from $z_1$, $z_3$, and $y$ would still be in the interior of triangle $z_1 z_2 z_3$. Thus, by continuity, if $y_3$ moves sufficiently close to edge $z_1 z_3$, the angle of $abcd$ incident to $y$ is convex as well.
}

The final possibility is that $abcd$ consists of one triangle outside $T$ and one triangle inside $T$.  We may assume without loss of generality that $abcd$ consists of triangle $z_1y_3y_2$ and an adjacent triangle inside $T$, see Figure~\ref{fig:4-gon-deg-4}(b).  We convexify the quadrilateral $z_1 y_3 y_1 y_2$, which necessarily also convexifies $abcd$.   The solution is to move $y_1$ towards $z_3$ to convexify the quadrilateral while the contents of triangle $T$ follow along linearly.   By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Handling $ac$-Inducing Vertices}

In this subsection we handle the fourth accommodating situation, namely when there is more than one $ac$-inducing vertex. 
We will show that we can convexify $abcd$ or reduce the problem size by one by performing at most two unidirectional morphs.


We first show that there can be at most two $ac$-inducing vertices.

\begin{lemma}  There are at most two $ac$-inducing vertices.
\end{lemma}
\begin{proof}
We show that there is at most one $ac$-inducing vertex on each side of the line $\overline{ac}$ through $a$ and $c$.
Suppose by way of contradiction that there are two  $ac$-inducing vertices $x$ and $x'$ on the same side of $\overline{ac}$. Since $x$ can be contracted to either $a$ or $c$, segment $ac$ lies inside $\Delta(x)$. However, $ac$ can not also lie inside $\Delta(x')$, so we have a contradiction. \end{proof}

Suppose there are two $ac$-inducing vertices, $x$ and $x'$ one on either side of $\overline{ac}$, and suppose that $x$ is on the same side of $\overline{ac}$ as $d$.  
See Figure~\ref{fig:problematic-ac-inducing}.

\begin{figure}[h]
  \centering
\includegraphics[width=1.5in]{fig/problematic-ac-inducing.pdf}
  \caption{Handling two $ac$-inducing vertices.}
  \label{fig:problematic-ac-inducing}
\end{figure}

Since $x$ is $ac$-inducing it must be $a$-contractible or $c$-contractible, say the former.  Then we can move $x$ close to $a$ and across the line $\overline{ac}$.  After moving $x$ to this position $x'$ is no longer $ac$-inducing since it can no longer be contracted to $a$ or to $c$.
Therefore $x'$ is now a non-problematic vertex of degree at most 5, and we can contract it to one of its neighbors and proceed recursively. 








==> quad-convexificationNew.tex <==
\section{Quadrilateral Convexification}
\label{sec:quad-convexification}

In this section we give an algorithm for Problem~\ref{prob:quad-convex}, to 
\update{morph a triangulation in order to convexify a quadrilateral}.
% by means of a morph composed of unidirectional morphing steps.  
The main result of the section is as follows:

%\begin{theorem*}{\bf [Reminder of Theorem~\ref{thm:quad-convex}.]}
%\quadconvex
%\end{theorem*}
\rephrase{Reminder of Theorem~\ref{thm:quad-convex}}{\quadconvex}

In the rest of this section we will prove Theorem~\ref{thm:quad-convex}. Recall that we have an $n$-vertex triangulation $\Gamma$ and a quadrilateral $abcd$ in $\Gamma$ with no vertex inside it and such that neither $ac$ nor $bd$ is an edge outside of $abcd$. Our goal is to morph $\Gamma$ so that $abcd$ becomes convex. We will show that Quadrilateral Convexification can be solved with one unidirectional morph.
%; our solution exploits a connection to the existence of hierarchical planar convex drawings of hierarchical planar triconnected graphs.

\update{
We first describe the main idea.
If $abcd$ is convex, we are done. Assume without loss of generality that $d$ is the reflex vertex of the non-convex quadrilateral, and thus $b$ is the tip of the arrowhead shape  (see Figure~\ref{fig:4-gon}).
The triangulation contains the edge $bd$.
Change the frame of reference so that $bd$ is horizontal.  (In fact, for technical reasons, we will need to make $bd$ slightly off from horizontal.) We will use one unidirectional morph that moves vertices along horizontal lines, i.e.~preserving their $y$-coordinates.   Our main tool will be a result about re-drawing a plane graph to have convex faces while keeping all vertices at the same $y$-coordinate---this is a result by Hong and Nagamochi expressed in terms of level planar drawings of hierarchical graphs.  We will then show that the linear motion from the original drawing to the new drawing in fact preserves planarity, and therefore is a unidirectional morph.  


\begin{figure}[h]
\label{fig:4-gon}
\centering
\includegraphics[width=1.2in]{fig/4-gon.pdf}
\caption{A non-convex quadrilateral $abcd$.}
\end{figure}


}


We introduce some definitions and terminology. A {\em hierarchical graph} is defined as a tuple $(G,\vec d,L,\gamma)$ where: 

\begin{itemize}
\item $G$ is a graph; 
\item $\vec d$ is an oriented straight line in the plane; 
\item $L$ is a set of parallel lines (sometimes called {\em layers}) that are orthogonal to $\vec d$; the lines in $L$ are assumed to be ordered in the same order as they are intersected by $\vec d$ when traversing such a line according to its orientation; and 
\item $\gamma$ is a function that maps each vertex of $G$ to a line in $L$ in such a way that, if an edge $(u,v)$ belongs to $G$, then $\gamma(u)\neq \gamma(v)$.
\end{itemize}

A {\em level drawing} of $(G,\vec d,L,\gamma)$ (sometimes also called {\em hierarchical drawing}) maps each vertex $v$ of $G$ to a point on the line $\gamma(v)$ and each edge $(u,v)$ of $G$ such that line $\gamma(u)$ precedes line $\gamma(v)$ in $L$ to an arc $\vec{uv}$ monotone with respect to $\vec d$. A {\em level planar drawing} of $(G,\vec d,L,\gamma)$ is a level drawing of $(G,\vec d,L,\gamma)$ in which no two curves representing edges of $G$ cross. A {\em straight-line convex level planar drawing} of $(G,\vec d,L,\gamma)$ is a level planar drawing of $(G,\vec d,L,\gamma)$ in which edges are represented by open straight-line segments between their end-vertices and faces are delimited by convex polygons.

A {\em hierarchical plane graph} is a hierarchical graph $(G,\vec d,L,\gamma)$ such that $G$ is a plane graph and such that a level planar drawing $\cal H$ of $(G,\vec d,L,\gamma)$ exists that ``respects'' the embedding of $G$ (that is, the planar drawing of $G$ in $\cal H$ belongs to the equivalence class corresponding to the planar embedding of $G$). 

Given a hierarchical plane graph $(G,\vec d,L,\gamma)$, an {\em st-face} of $G$ is a face delimited by two paths $(s=u_1,u_2,\dots,u_k=t)$ and $(s=v_1,v_2,\dots,v_l=t)$ such that $\gamma(u_i)$ precedes $\gamma(u_{i+1})$ in $L$, for every $1\leq i\leq k-1$, and such that $\gamma(v_i)$ precedes $\gamma(v_{i+1})$ in $L$, for every $1\leq i\leq l-1$.  We say that $(G,\vec d,L,\gamma)$ is a {\em hierarchical plane st-graph} if every face of $G$ is an st-face.

A straight line segment directed from a point $x$ to a point $y$ is \emph{monotone} with respect to an oriented straight line $\vec d$ if the projection of $x$ on $\vec d$ precedes the projection of $y$ on $\vec d$ according to the orientation of $\vec d$. A path $P= (u_1, \dots, u_n)$ drawn with straight-line segments is \emph{$\vec d$-monotone} if the straight-line segment oriented from $u_i$ to $u_{i+1}$ is monotone with respect to $\vec d$, for $i=1, \dots, n-1$; a polygon $Q$ is \emph{$\vec d$-monotone} if it contains two vertices $s$ and $t$ such that the two paths between $s$ and $t$ that delimit $Q$ are both $\vec d$-monotone. 

Let $\cal H$ be any straight-line level planar drawing of a hierarchical plane graph $(G,\vec d,L,\gamma)$ and let $f$ be a face of $G$; then, it is easy to argue that $f$ is an st-face if and only if the polygon delimiting $f$ in $\cal H$ is $\vec d$-monotone. We will also exploit the following two simple lemmata.

\begin{lemma}\label{le:convex-is-monotone}
Any convex polygon $Q$ is $\vec d$-monotone, for any oriented straight line $\vec d$ in the plane which is not perpendicular to any straight line through two vertices of $Q$. 
\end{lemma}

\begin{proof}
\update{I DON'T THINK THIS PROOF NEEDS TO BE SO LONG.  AL.}
Refer to Fig.~\ref{fig:convex-is-monotone}. Denote by $u_1,\dots,u_k$ the vertices of $Q$, in any order. Let $\vec d$ be any oriented straight line not perpendicular to any straight line through two vertices of $Q$. For $1\leq i\leq k$, let $u'_i$ be the projection of $u_i$ on $\vec d$. Since $Q$ is convex and $\vec d$ is not perpendicular to any straight line through two vertices of $Q$, we have that $u'_i$ and $u'_j$ are distinct, for $1\leq i\neq j \leq k$. Let $\sigma$ be the total order of the projections $u'_i$ as they are encountered when traversing $\vec d$ according to its orientation. Let $u'_a$ and $u'_b$ be the first and the last element in $\sigma$, respectively. We claim that the two paths $P_1$ and $P_2$ connecting $u_a$ and $u_b$ along $Q$ are $\vec d$-monotone. The claim directly implies the lemma.

\begin{figure}[htb]
\begin{center}
\includegraphics[scale=0.55]{fig/convex-is-monotone}
\caption{Illustration for the proof of Lemma~\ref{le:convex-is-monotone}.}
\label{fig:convex-is-monotone}
\end{center}
\end{figure}

We prove the claim by induction on $k$. If $k=3$, then the claim is trivially proved. If $k \geq 4$, then let $u'_c$ be the second element in $\sigma$. Assume, w.l.o.g., that $u_c$ is in $P_1$. Then, let $Q'$ be the convex polygon obtained from $Q$ by inserting a segment connecting $u_c$ with the second vertex of $P_2$, say $u_d$, and by removing $u_a$ and its two incident segments. Let $\sigma'=\sigma\setminus\{u'_a\}$. By assumption, $u'_c$ and $u'_b$ are the first and the last element in $\sigma'$, respectively. By induction, the two paths $P'_1=P_1\setminus\{(u_a,u_c)\}$ and $P'_2=P_2\setminus\{(u_a,u_d)\}\cup\{u_c,u_d\}$ are $\vec d$-monotone. Finally, the straight line segments directed from $u_a$ to $u_c$ and to $u_d$ are monotone with respect to $\vec d$, given that $u'_a$ is the first element in $\sigma$. Hence, paths $P_1$ and $P_2$ are $\vec d$-monotone and polygon $Q$ is $\vec d$-monotone.
\end{proof}

\begin{lemma} \label{le:monotone-in-one-direction}
Any planar polygon $Q$ with $4$ vertices is $\vec d$-monotone, for some oriented straight line $\vec d$ in the plane.
\end{lemma} 

\begin{proof}
If $Q$ is convex, then the statement follows by Lemma~\ref{le:convex-is-monotone}. Otherwise, assume that $Q$ consists of vertices $x$, $y$, $w$, and $z$ in this clockwise order around $Q$, and assume that the angle internal to $Q$ and incident to $x$ is larger than $\pi$ radians. Consider a straight line orthogonal to segment $xw$ and orient it in any way. Denote by $\vec d$ the resulting oriented straight line. Then $Q$ consists of two paths which are monotone with respect to $\vec d$; these two paths are either $ywz$ and $yxz$, or $zwy$ and $zxy$. \end{proof}

We will use an algorithm by Hong and Nagamochi that constructs convex straight-line level planar drawings of hierarchical plane st-graphs~\cite{hn-cdhpgcpg-10}. Here we explicitly formulate a weaker version of their main theorem.\footnote{We make some remarks. First, the main result in~\cite{hn-cdhpgcpg-10} proves that a convex straight-line level planar drawing of $(G,\vec d,L,\gamma)$ exists even if a convex polygon representing the cycle delimiting the outer face of $G$ is arbitrarily prescribed. Second, the result holds for a super-class of the $3$-connected planar graphs, namely for all the graphs that admit a convex straight-line drawing~\cite{cyn-lacdp-84,t-prg-84}. Third, the result assumes that the lines in $L$ are horizontal; however, a suitable rotation of the coordinate axes shows how that assumption is not necessary. Fourth, looking at the figures in~\cite{hn-cdhpgcpg-10} one might get the impression that the lines in $L$ need to be equidistant; however, this is nowhere used in their proof, hence the result holds for any set of parallel lines.}

\begin{theorem} \label{th:hong-nagamochi} (Hong and Nagamochi~\cite{hn-cdhpgcpg-10})
Every $3$-connected hierarchical plane st-graph $(G,\vec d,L,\gamma)$ admits a convex straight-line level planar drawing.
\end{theorem}

Consider any straight-line level planar drawing $\cal H$ of a hierarchical plane graph $(G,\vec d,L,\gamma)$. Since each edge $(u,v)$ of $G$ is represented in $\cal H$ by a $\vec d$-monotone arc, the fact that $(u,v)$ intersects a line $l_i\in L$ does not depend on the actual drawing $\cal H$, but only on the fact that $l_i$ lies between lines $\gamma(u)$ and $\gamma(v)$ in $L$. Assume that each line $l_i\in L$ is oriented so that $\vec d$ cuts $l_i$ from the right to the left of $l_i$. We say that an edge $e$ {\em precedes} ({\em follows}) a vertex $v$ on a line $l_i$ in $\cal H$ if $\gamma(v)=l_i$, $e$ intersects $l_i$ in a point $p_i(e)$, and $p_i(e)$ precedes (resp. follows) $v$ on $l_i$ when traversing such a line according to its orientation. Also, we say that an edge $e$ {\em precedes} ({\em follows}) an edge $e'$ on a line $l_i$ in $\cal H$ if $e$ and $e'$ both intersect $l_i$ at points $p_i(e)$ and $p_i(e')$, and $p_i(e)$ precedes (resp. follows) $p_i(e')$ on $l_i$ when traversing such a line according to its orientation.

Now consider two straight-line level planar drawings ${\cal H}_1$ and ${\cal H}_2$ of a hierarchical plane graph $(G,\vec d,L,\gamma)$. We say that ${\cal H}_1$ and ${\cal H}_2$ are {\em left-to-right equivalent} if, for any line $l_i\in L$, for any vertex or edge $x$ of $G$, and for any vertex or edge $y$ of $G$, we have that $x$ precedes (follows) $y$ on $l_i$ in ${\cal H}_1$ if and only if $x$ precedes (resp. follows) $y$ on $l_i$ in ${\cal H}_2$. We are going to make use of the following lemma.

\begin{lemma} \label{le:unidirectional}
Let ${\cal H}_1$ and ${\cal H}_2$ be two left-to-right equivalent straight-line level planar drawings of the same hierarchical plane graph $(G,\vec d,L,\gamma)$. Then the linear morph \mmorph{{\cal H}_1,{\cal H}_2} transforming ${\cal H}_1$ into ${\cal H}_2$ is planar and unidirectional.
\end{lemma}

\begin{proof}
\red{MISSING PROOF HERE}
\end{proof}

We are now ready to prove Theorem~\ref{thm:quad-convex} and hence to solve the Quadrilateral Convexification problem with one unidirectional morph. First, observe that in the triangulation $\Gamma$, either $ac$ or $bd$ is an edge lying inside quadrilateral $abcd$; this comes from the fact that $\Gamma$ is a planar straight-line drawing of a maximal planar graph $G$. Assume without loss of generality that $ac$ is an edge lying inside quadrilateral $abcd$ and recall that, by the assumption of the Quadrilateral Convexification problem, $bd$ is not an edge of $G$.

Remove edge $ac$ from $\Gamma$ obtaining a planar straight-line drawing $\Gamma'$ of a planar graph $G'$. We have the following. 

\red{FIGURES TO BE DRAWN AGAIN}
\begin{figure}[t]
\begin{center}
\begin{tabular}{c c c}
\includegraphics[width=0.3\textwidth]{fig/Fast-Convexifier-1-bis.pdf} \hspace{1mm} &
\includegraphics[width=0.3\textwidth]{fig/Fast-Convexifier-4-bis.pdf} \hspace{1mm} &
\includegraphics[width=0.3\textwidth]{fig/Fast-Convexifier-5-bis.pdf} \\
(a) \hspace{1mm} & (b) \hspace{1mm} & (c)
\end{tabular}
\caption{(a) Straight-line planar drawing $\Gamma$ of $G$. (b) Straight-line level planar drawing $\Gamma'$ of $(G',\vec d,L',\gamma')$. (c) Convex straight-line level planar drawing $\Gamma'_M$ of $(G',\vec d,L',\gamma')$.}
\label{fig:convexifier-process}
\end{center}
\end{figure}

\begin{lemma} \label{le:triconnected-after-removal}
Graph $G'$ is $3$-connected.
\end{lemma}

\begin{proof}
\red{MISSING PROOF HERE}
\end{proof}

Consider the polygon $abcd$ in $\Gamma$ and in $\Gamma'$. By Lemma~\ref{le:monotone-in-one-direction}, $abcd$ is $\vec d$-monotone, for some oriented straight line $\vec d$. Slightly perturb the slope of $\vec d$ so that no line through two vertices of $G$ in $\Gamma$ is perpendicular to $\vec d$. If the perturbation is small enough, then $abcd$ is still $\vec d$-monotone.
%
Denote by $u_1,\dots,u_{n-1}$ the vertices of $G'$ ordered according to their projection on $\vec d$. For $1\leq i\leq n-1$, denote by $l_i$ the line through $u_i$ orthogonal to $\vec d$. Let $L'=\{l_1,\dots,l_{n-1}\}$; note that the lines in $L'$ are parallel and distinct. Let $\gamma'$ be the function that maps $u_i$ to $l_i$, for $1\leq i\leq n-1$. See Fig.~\ref{fig:convexifier-process}(b).

\begin{lemma} \label{le:orientation}
$(G',\vec d,L',\gamma')$ is a hierarchical plane st-graph.
\end{lemma}
%
\begin{proof}
By construction, $\Gamma'$ is a straight-line level planar drawing of $(G',\vec d,L',\gamma')$, hence $(G',\vec d,L',\gamma')$ is a hierarchical plane graph. 

Further, every polygon delimiting a face of $G'$ in $\Gamma'$ is $\vec d$-monotone. This is true for $abcd$ by construction and for every other polygon $Q_i$ delimiting a face of $G'$ in $\Gamma'$ by Lemma~\ref{le:convex-is-monotone}, given that $Q_i$ is a triangle (hence it is convex) and given that no line through two vertices of $G$ in $\Gamma$ is perpendicular to $\vec d$ (by construction). Since every polygon delimiting a face of $G'$ in $\Gamma'$ is $\vec d$-monotone, every face of $G'$ is an st-face, hence $(G',\vec d,L',\gamma')$ is a hierarchical plane st-graph.
\end{proof}

By Lemmata~\ref{le:triconnected-after-removal} and~\ref{le:orientation}, $(G',\vec d,L',\gamma')$ is a $3$-connected hierarchical plane st-graph. By Theorem~\ref{th:hong-nagamochi}, a convex straight-line level planar drawing $\Gamma'_M$ of $(G',\vec d,L',\gamma')$ exists. In particular, polygon $abcd$ is convex in $\Gamma'_M$. Observe that it might be the case that the angle incident to one of $a$, $b$, $c$, and $d$ (say at $b$) inside $\Gamma'_M$ is $\pi$ radians, that is, $abcd$ is convex but not strictly-convex. A slight perturbation of the position of $b$ along $\gamma(b)$ is however sufficient to modify $\Gamma'_M$ so that $abcd$ is strictly-convex.



%Denote by $r$ and $s$ the minimum and the maximum index such that $u_r$ and $u_s$ belong to $C_v$, respectively. Denote by $l(v)$ the line through $v$ orthogonal to $\vec d$ in $\Gamma$. If $l(v)$ were contained in the half-plane delimited by $l_r$ and not containing $l_s$, then $v$ would not lie inside $Q_v$ in $\Gamma$, as the projection of every vertex of $Q_v$ on $\vec d$ would follow the projection of $v$ on $\vec d$. Analogously, $l(v)$ is not contained in the half-plane delimited by $l_s$ and not containing $l_r$. It follows that $l(v)$ is ``in-between'' $l_r$ and $l_s$, that is, $l(v)$ lies in the strip defined by $l_r$ and $l_s$.
%
Construct a straight-line planar drawing $\Gamma_M$ of $G$ from $\Gamma'_M$ by drawing edge $ac$ as an open straight-line segment. Since $abcd$ is strictly-convex, this introduces no crossing in the drawing.

\red{FIGURES TO BE DRAWN AGAIN}
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\textwidth]{fig/Fast-Convexifier-6.pdf}
\caption{Morphing $\Gamma$ into a straight-line planar drawing $\Gamma_M$ of $G$ in which the polygon $Q^M_v$ representing $C_v$ is convex. The thick line parallel to $l_i$ is $l(v)$.}
\label{fig:convexifier-morphing}
\end{center}
\end{figure}

Problem Quadrilateral Convexification can then be solved via a single linear morph $\langle \Gamma,\Gamma_M \rangle$ transforming $\Gamma$ into $\Gamma_M$. See Fig.~\ref{fig:convexifier-morphing}. Note that $\Gamma$ and $\Gamma_M$ are left-to-right equivalent straight-line level planar drawings of $(G,\vec d,L,\gamma)$, hence, by Lemma~\ref{le:unidirectional}, $\langle \Gamma,\Gamma_M \rangle$ is unidirectional and planar.

























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\remove{
Suppose the triangular outer boundary of the drawing is $z_1z_2z_3$.  
If $abcd$ is convex, we are done. Assume without loss of generality that $d$ is the reflex vertex of the non-convex quadrilateral, and thus $b$ is the tip of the arrowhead shape  (see Figure~\ref{fig:4-gon}).
The triangulation contains the edge $bd$.

\begin{figure}[h]
\label{fig:4-gon}
\centering
\includegraphics[width=1.2in]{fig/4-gon.pdf}
\caption{A non-convex quadrilateral $abcd$.}
\end{figure}

We follow Cairns's idea of reducing the size of the problem by one by contracting a non-boundary vertex $v$ with $\Deg(v)\le5$ to a neighbor, recursively solving the problem on the smaller graph, and then uncontracting $v$.
We will find a pseudomorph whose morphing steps are unidirectional and rely on Theorem~\ref{thm:pseudomorph} to convert the pseudomorph to a morph with the same number of unidirectional morphing steps.

A planar graph always has a vertex $v$ of degree at most 5, but not all such vertices are useful for our purposes.
In particular, we must keep the outer boundary fixed,  
we must not ``destroy'' quadrilateral $abcd$, and we must not introduce the edge $ac$ when we contract $v$, since the external chord $ac$ would preclude convexification of $abcd$. 
%We will distinguish the \emph{non-problematic} vertices whose contraction preserves the properties we need.  More precisely, 
Formally, we define a vertex $v$ to be \emph{problematic} if:
\begin{itemize}
  \item  $v$ is a boundary vertex (one of $z_1,z_2,z_3$),
  \item $v$ is a quadrilateral vertex (one of $a,b,c,d$), or
  \item $v$ is $ac$-\emph{inducing}, that is, $v$ has degree at most 5, $v$ is not a boundary or quadrilateral vertex, $v$ is adjacent to both $a$ and $c$, and $v$ is $a$-contractible or $c$-contractible.  
  (We use the term ``$ac$-inducing'' because contracting $v$ to $a$ or $c$ would introduce edge $ac$.)
\end{itemize}

If there is a non-problematic vertex $v$ of degree at most 5 then we contract $v$ to a neighbor, recursively solve the quadrilateral convexification problem in the smaller graph, and then uncontract $v$.  
By Theorem~\ref{thm:pseudomorph} we can convert this pseudomorph to a morph with the same number of unidirectional morphing steps. 
The total number of unidirectional morphing steps then satisfies $S(n) = S(n-1) + O(1)$, which solves to $S(n) \in O(n)$. 

It remains to deal with the case where all vertices of degree at most 5 are problematic.  
We will show that we can find a constant number of unidirectional morphing steps that either convexify the quadrilateral $abcd$ or reduce the problem size.  

Formally, we say that a triangulation is \emph{accommodating} if we have one of the following:
\begin{enumerate}
\item a non-problematic vertex of degree at most 5,
\item a vertex of the quadrilateral that is not on the boundary and has degree at most 4, 
\item a boundary vertex of degree 3 or three boundary vertices of degree 4, or
\item more than one $ac$-inducing vertex.
\end{enumerate}

In the subsections below we show how to handle each of the accommodating situations.  (We already know how to handle the first situation.) 
Theorem~\ref{thm:quad-convex} then follows from a counting argument that shows that every triangulation is accommodating:

\begin{lemma} Every triangulation is accommodating.
\label{lem:accommodating}
\end{lemma}
\begin{proof}
Define the \emph{value} of a vertex $v$ to be $6 - \Deg(v)$.  Because the number of edges in a triangulation is $3n-6$, the total value of all vertices is $6n - \sum_v \Deg(v) = 12$.

Suppose the triangulation is not accommodating. Then the three boundary vertices have degrees at least $4$, $4$, and $5$, i.e.~total value at most $5$.  
Any vertex of the quadrilateral that is not on the boundary has degree at least $5$, so the total value of the quadrilateral non-boundary vertices is at most $4$.  There can be at most one $ac$-inducing vertex $v$, and it cannot have degree 3 otherwise its 3 neighbors would be connected, and therefore $ac$ would be an edge, violating our assumption.  This implies that the total value of $ac$-inducing vertices is at most 2. 
All other vertices have degree at least 6, hence value at most 0.  
Thus, the total value of all vertices is at most 11, a contradiction.
\end{proof}


We now discuss the running time of the algorithm to compute the morph for Quadrilateral Convexification.  
At each step we find a vertex to contract, recursively find a morph of the smaller graph, and then appeal to Theorem~\ref{thm:pseudomorph} to convert the resulting pseudomorph to a morph with the same number of unidirectional morphing steps.  The number of unidirectional morphs is always $O(n)$.  Each time we convert a pseudomorph to a morph, this takes $O(n)$ time (by Theorem~\ref{thm:pseudomorph}).  Thus, the time spent on pseudomorph conversion alone is $T(n) = T(n-1) + O(n)$, which solves to $T(n) \in O(n^2)$.  
We also need to find the vertex to contract or the accommodating situation, and decide how to handle it (with details below).  It is easy to see that in each step this can be accomplished in $O(n)$ time.
%In fact this can probably be reduced to $O(n)$ in total, though such a reduction is irrelevant to the total time bound.
Thus the total running time is $O(n^2)$. 

  
\remove{
As for the work to find the morph, we order the vertices by degree.  We can update this order in constant time per contraction, since we only contract vertices of degree at most 5.
We perform a linear search through the vertices of degree at most 5. 
We can test in constant time if a vertex is problematic.  There are at most 8 problematic vertices: 4 quadrilateral vertices, 3 boundary vertices, and (by Lemma~\ref{}) at most 1 $ac$-inducing vertex.
We can test in constant time if we have an accommodating situation.   
In the subsections below, we show that  each accommodating situation can be dealt with in constant time.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Handling Quadrilateral Vertices}

In this subsection we handle the second accommodating situation, namely when there is a vertex of the quadrilateral that is not on the boundary and has degree at most 4.  We will show that we can convexify $abcd$ or reduce the problem size by one by moving one vertex in a straight line, which is a unidirectional morph.

We consider the vertices of the quadrilateral in turn.
Suppose vertex $a$ has degree at most 4 and is not a boundary vertex.  
See Figure~\ref{fig:problematic-quad-a}.
%
\begin{figure}[htb]
\centering
\def\sf{1.4}
\hfill\subfigure[]{\includegraphics[scale=\sf]{fig/problematic-quad-a.pdf}\label{fig:problematic-quad-a}}\hfill
\subfigure[]{\includegraphics[scale=\sf]{fig/problematic-quad-b.pdf}\label{fig:problematic-quad-b}}\hfill
\caption{\subref{fig:problematic-quad-a} Handling vertex $a$. 
\subref{fig:problematic-quad-b}~Handling vertex $b$. 
}
\end{figure}
%
\remove{
\begin{figure}[h]
  \centering
\includegraphics[width=1.5in]{fig/problematic-quad-a.pdf}
  \caption{Handling vertex $a$. }
  \label{fig:problematic-quad-a}
\end{figure}
}
Observe the following fact: in any triangle or quadrilateral, every edge must be incident to at least one vertex that lies in the kernel. Applying this fact to $\Delta(a)$ shows that $b$ or $d$ must be in the kernel of $\Delta(a)$.  
We can thus move $a$ to within a small distance from whichever vertex is in the kernel to directly convexify $abcd$.


The case when vertex $c$ has degree at most 4 and is not a boundary vertex is symmetric.

Next suppose that $b$ has degree at most 4 and is not a boundary vertex. 
See Figure~\ref{fig:problematic-quad-b}.
Then $b$ must have exactly one neighbor $x$ that is not on $abcd$, and $x$ must be adjacent to both $a$ and $c$.  Since $d$ is a reflex vertex of the quadrilateral $\Delta(b)=axcd$, vertex $x$ must be in the kernel of $\Delta(b)$.  So we contract $b$ to $x$, recursively convexify $axcd$, and uncontract $b$.

\remove{
\begin{figure}[h]
  \centering
\includegraphics[width=1.5in]{fig/problematic-quad-b.pdf}
  \caption{Handling vertex $b$.}
  \label{fig:problematic-quad-b}
\end{figure}
}


Finally, suppose that $d$ has degree at most 4 and is not a boundary vertex.
See Figure~\ref{fig:problematic-quad-d}~(a) and~(b).
Note that $d$ cannot have degree 3 because $ac$ is not an edge.  
Thus $d$ must have exactly one neighbor $x$ that is not on $abcd$ and $x$ must be adjacent to $a$ and $c$. 
If $x$ is outside the triangle $abc$ then $a$ and $c$ are in the kernel of $\Delta(d)$, so we can directly convexify $abcd$ by moving $d$ to within a small distance from $a$.
Otherwise we contract $d$ to $x$, recursively convexify $abcx$, and uncontract $d$. 


\begin{figure}[h]
  \centering
\includegraphics[width=3in]{fig/problematic-quad-d.pdf}
  \caption{Handling vertex $d$.}
  \label{fig:problematic-quad-d}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Handling Boundary Vertices}

In this subsection we handle the third accommodating situation, namely when there is a boundary vertex of degree 3 or three boundary vertices of degree 4.
We will show that a single unidirectional morph suffices to convexify $abcd$ or reduce the problem size.


In all the cases so far, we moved one vertex at a time.
To handle boundary vertices we will move one vertex of a triangle along a straight line and have the vertices inside the triangle follow along linearly. By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph.

Suppose boundary vertex $z_1$ has degree 3. 
See Figure~\ref{fig:4-gon-deg-3}~(a).
\begin{figure}[h]
\label{fig:4-gon-deg-3}
\centering
\includegraphics[width=4.5in]{fig/4-gon-deg-3.pdf}
\caption{Handling a boundary vertex of degree 3.}
\end{figure}

Then $z_1$ must have a neighbor $y$ that is adjacent to $z_2$ and $z_3$.  If $abcd$ lies entirely inside the triangle $T=yz_2z_3$ then we recursively morph the subgraph contained in $T$.  Otherwise $abcd$ must include at least one triangle outside $T$.  It cannot have both its triangles outside $T$ by the assumption that there is no edge $ac$.  Thus we can assume without loss of generality that $abcd$ consists of triangle $z_1yz_3$ and an adjacent triangle formed by $z_3 y$ and an internal vertex of $T$, see Figure~\ref{fig:4-gon-deg-3}(b).  
%The solution is to move $y$ towards $z_1$ to directly convexify $abcd$.  As $y$ is moved, the contents of triangle $T$ follow along linearly.  By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph. 
The solution is to move $y$ towards an interior point of the edge $z_1 z_2$ to directly convexify the quadrilateral.  As $y$ is moved, the contents of triangle $T$ follow along linearly.  By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph.   Note that this motion will convexify the quadrilateral since every interior point of $T$ is a convex combination of $y$, $z_2$, and $z_3$ with a positive contribution from $z_3$.

Now suppose that all three boundary vertices have degree 4.  See Figure~\ref{fig:4-gon-deg-4}(a).
In this case there exists an internal triangle $T= y_1 y_2 y_3$ containing all the internal vertices with 
$y_i$ adjacent to $z_j$ for $j \ne i$ with $i,j \in \{1,2,3\}$. 
\begin{figure}[h]
\centering
\includegraphics[width=4.5in]{fig/4-gon-deg-4.pdf}
\caption{Handling the case of three boundary vertices of degree 4.}
\label{fig:4-gon-deg-4}
\end{figure}
%$y_1$ adjacent to $z_2, z_3$ and $y_2$ adjacent to $z_3,z_1$ and $y_3$ adjacent to $z_1, z_2$.   
If $abcd$ lies entirely inside $T$ then we recursively morph the subgraph contained in $T$.  If $abcd$ lies entirely outside $T$ then without loss of generality $abcd$ is $z_1y_3y_2z_3$. The solution is to move $y_3$ towards $z_1$ to directly convexify the
quadrilateral. As $y_3$ is moved, the contents of triangle $T$ follow along linearly.
\remove{  -- Fabrizio's change is below, but I think it belongs with the previous case.  A.L.
The solution is to move $y_3$ 
towards an interior point of edge $z_1 z_3$ to directly convexify the quadrilateral.
%to within a small distance of $z_1$ and perturb it to directly convexify the 4-gon.  
As $y_3$ is moved, the contents of triangle $T$  follow along linearly.  By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph. Note that, if $y_3$ moves sufficiently close to edge $z_1 z_3$, quadrilateral $abcd$ does become convex. Indeed, if $y_3$ moved {\em on} an interior point of edge $z_1 z_3$, then the angle of $abcd$ incident to $y$ would be convex, since the vertex of $abcd$ different from $z_1$, $z_3$, and $y$ would still be in the interior of triangle $z_1 z_2 z_3$. Thus, by continuity, if $y_3$ moves sufficiently close to edge $z_1 z_3$, the angle of $abcd$ incident to $y$ is convex as well.
}

The final possibility is that $abcd$ consists of one triangle outside $T$ and one triangle inside $T$.  We may assume without loss of generality that $abcd$ consists of triangle $z_1y_3y_2$ and an adjacent triangle inside $T$, see Figure~\ref{fig:4-gon-deg-4}(b).  We convexify the quadrilateral $z_1 y_3 y_1 y_2$, which necessarily also convexifies $abcd$.   The solution is to move $y_1$ towards $z_3$ to convexify the quadrilateral while the contents of triangle $T$ follow along linearly.   By Lemma~\ref{lemma:convex-comb} this is a unidirectional morph.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Handling $ac$-Inducing Vertices}

In this subsection we handle the fourth accommodating situation, namely when there is more than one $ac$-inducing vertex. 
We will show that we can convexify $abcd$ or reduce the problem size by one by performing at most two unidirectional morphs.


We first show that there can be at most two $ac$-inducing vertices.

\begin{lemma}  There are at most two $ac$-inducing vertices.
\end{lemma}
\begin{proof}
We show that there is at most one $ac$-inducing vertex on each side of the line $\overline{ac}$ through $a$ and $c$.
Suppose by way of contradiction that there are two  $ac$-inducing vertices $x$ and $x'$ on the same side of $\overline{ac}$. Since $x$ can be contracted to either $a$ or $c$, segment $ac$ lies inside $\Delta(x)$. However, $ac$ can not also lie inside $\Delta(x')$, so we have a contradiction. \end{proof}

Suppose there are two $ac$-inducing vertices, $x$ and $x'$ one on either side of $\overline{ac}$, and suppose that $x$ is on the same side of $\overline{ac}$ as $d$.  
See Figure~\ref{fig:problematic-ac-inducing}.

\begin{figure}[h]
  \centering
\includegraphics[width=1.5in]{fig/problematic-ac-inducing.pdf}
  \caption{Handling two $ac$-inducing vertices.}
  \label{fig:problematic-ac-inducing}
\end{figure}

Since $x$ is $ac$-inducing it must be $a$-contractible or $c$-contractible, say the former.  Then we can move $x$ close to $a$ and across the line $\overline{ac}$.  After moving $x$ to this position $x'$ is no longer $ac$-inducing since it can no longer be contracted to $a$ or to $c$.
Therefore $x'$ is now a non-problematic vertex of degree at most 5, and we can contract it to one of its neighbors and proceed recursively. 
}






